Praxis: Distilling Physical Interaction Priors from Egocentric Videos for Generalizable Whole-Body Manipulation

Mobile humanoid manipulation requires both reaching a usable workspace and preserving precise hand-object interactions as object poses and contact conditions change. Learning these behaviors from limited task-specific data remains challenging. To bridge this gap, we introduce Praxis, a whole-body manipulation framework that combines physical interaction priors from one-shot egocentric video demonstrations with closed-loop posture calibration and online perception. The framework coordinates three stages: vision-language-guided navigation toward target objects, closed-loop posture calibration to align the arm-hand workspace, and dexterous manipulation with synchronized upper- and lower-body control. Online visual feedback re-grounds demonstrated interaction geometry under new object poses and scene configurations, while tactile feedback adapts hand motions to actual contact conditions. Each manipulation skill is specified by one human demonstration, without task-specific manipulation-policy retraining. Experiments across five long-horizon manipulation tasks demonstrate spatial, visual, and cross-object generalization, as well as recovery from external physical disturbances across all three stages.

==> teaser.tex <==
% Original first appendix figure, placed after the title as Figure 1.
% The PDF CropBox excludes blank canvas; the underlying artwork is unchanged.
\makeatletter
\newcommand{\PraxisTeaser}{%
\begin{minipage}{\textwidth}
\centering
\includegraphics[width=0.8\textwidth,pagebox=cropbox]{teaser1.pdf}
\begingroup
\def\@captype{figure}
\vspace{-0.05in}
\caption{\Method{} is a hierarchical whole-body manipulation framework that learns generalizable and robust policies from human egocentric videos. Five tasks are shown from top to bottom: \texttt{Pour Water}, \texttt{Hand Over}, \texttt{Pull Drawer}, \texttt{Manipulate Pipette}, \texttt{Open Lid}.}
\label{fig:teaser}
\endgroup
\end{minipage}
\par\vspace{8pt}
}
\IEEEaftertitletext{\PraxisTeaser}
\makeatother

